Scaling Graph-Based Dependency Parsing with Arc Vectorization and Attention-Based Refinement

We propose a novel architecture for graph-based dependency parsing that explicitly constructs vectors, from which both arcs and labels are scored. Our method addresses key limitations of the standard two-pipeline approach by unifying arc scoring and labeling into a single network, reducing scalability issues caused by the information bottleneck and lack of parameter sharing. Additionally, our architecture overcomes limited arc interactions with transformer layers to efficiently simulate higher-order dependencies. Experiments on PTB and UD show that our model outperforms state-of-the-art parsers in both accuracy and efficiency.

==> img/parsing_speed.tex <==
\begin{figure}[t]
  \centering
  \small
\hspace{-30pt}\begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=0.5cm,
        ylabel={sents/sec},
        xtick={0.2, 1.4, 2.6, 3.8},
        xticklabels={\node[align=center]{Loc};, \node[align=center]{ArcLoc};, \node[align=center]{ArcLoc\\1 Transf. Layer};, \node[align=center]{CRF2o};},
        ymin=0,
        ymax=550,
        nodes near coords,
        nodes near coords align={vertical},
        enlarge x limits=0.5,
        font=\rmfamily,
        title style={font=\rmfamily},
        every axis label/.append style={font=\rmfamily},
        every tick label/.append style={font=\rmfamily},
        title={},
        xlabel style={align=center},
        ]
        \addplot[fill=cyan!10] coordinates {(0.8,465)};
        \addplot[fill=cyan!10] coordinates {(1.6,454)};
        \addplot[fill=cyan!10] coordinates {(2.4,439)};
        \addplot[fill=cyan!10] coordinates {(3.2,306)};
    \end{axis}
\end{tikzpicture}
  \vspace*{12pt} \caption{Parsing speed on PTB in sent/s.}
  \label{fig:speed}
\end{figure}


==> tables/PTB_DEV_Loc_ArcLoc.tex <==
\begin{table}[H]
  \centering
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{lllllrrr}
  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{r}{\# Param ($10^{6}$)} & UAS & LAS \\
  \midrule
\multicolumn{5}{l}{\textsc{Loc}}                    & \multicolumn{1}{r}{4}   & \multicolumn{1}{r}{96.85}      & 95.16        \\
\multicolumn{5}{l}{\textsc{CRF2o}}                  & \multicolumn{1}{r}{4}   & \multicolumn{1}{r}{96.87}      & 95.18        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 0 Transf. layer} & \multicolumn{1}{r}{4}   & \multicolumn{1}{r}{96.85}      & 95.16        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 1 Transf. layer} & \multicolumn{1}{r}{4}   & \multicolumn{1}{r}{96.84}      & 95.13        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 2 Transf. layer} & \multicolumn{1}{r}{4}   & \multicolumn{1}{r}{96.81}      & 95.12        \\
\multicolumn{5}{l}{\textsc{Loc}}                    & \multicolumn{1}{r}{50}  & \multicolumn{1}{r}{96.83}      & 95.16        \\
\multicolumn{5}{l}{\textsc{CRF2o}}                  & \multicolumn{1}{r}{50}  & \multicolumn{1}{r}{96.89}      & 95.19        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 0 Transf. layer} & \multicolumn{1}{r}{50}  & \multicolumn{1}{r}{96.91}      & 95.26        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 1 Transf. layer} & \multicolumn{1}{r}{50}  & \multicolumn{1}{r}{96.90}      & 95.22        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 2 Transf. layer} & \multicolumn{1}{r}{50}  & \multicolumn{1}{r}{96.87}      & 95.20        \\
\multicolumn{5}{l}{\textsc{Loc}}                    & \multicolumn{1}{r}{100} & \multicolumn{1}{r}{96.79}      & 95.12        \\
\multicolumn{5}{l}{\textsc{CRF2o}}                  & \multicolumn{1}{r}{100} & \multicolumn{1}{r}{96.88}      & 95.18        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 0 Transf. layer} & \multicolumn{1}{r}{100} & \multicolumn{1}{r}{96.92}      & 95.29        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 1 Transf. layer} & \multicolumn{1}{r}{100} & \multicolumn{1}{r}{96.91}      & 95.23        \\
\multicolumn{5}{l}{\textsc{ArcLoc} 2 Transf. layer} & \multicolumn{1}{r}{100} & \multicolumn{1}{r}{96.90}      & 95.22        \\
\end{tabular}
\end{adjustbox}
\caption{Impact of arc vectors and Transformers on PTB dev data.}\label{tab:trans}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

